Change-point detection in high-dimensional covariance structure

In this paper we introduce a novel approach for an important problem of break detection. Specifically, we are interested in detection of an abrupt change in the covariance structure of a high-dimensional random process -- a problem, which has applications in many areas e.g., neuroimaging and finance. The developed approach is essentially a testing procedure involving a choice of a critical level. To that end a non-standard bootstrap scheme is proposed and theoretically justified under mild assumptions. Theoretical study features a result providing guaranties for break detection. All the theoretical results are established in a high-dimensional setting (dimensionality $p \gg n$). Multiscale nature of the approach allows for a trade-off between sensitivity of break detection and localization. The approach can be naturally employed in an on-line setting. Simulation study demonstrates that the approach matches the nominal level of false alarm probability and exhibits high power, outperforming a recent approach.

==> 4thmoment.tex <==
\begin{lemma}\label{OmegaDelta}
	Let \ref{subGaussianElements} holds. 
	
	\begin{equation}
	\Prob{\infnorm{\Omega^* - \hat{\Omega}} \ge \omegaDelta } \le \probOmegaBound \coloneqq  2ps\ex{-x^2/(2K^2\sigma^2_{\max})} + p^4e^{-t}
	\end{equation}
	
	\begin{equation}
	\omegaDelta \coloneqq \Bernstain{x^4+\abs{\omega_{\ione, \itwo, \ithree, \ifour}}}{t}{s}{\sigma^2_{4\max}} 
	\end{equation}
	
\end{lemma}

\begin{proof}
	Due to sub-Gaussianity one can bound elements of $X_i$ with high probability: 
	
	\begin{equation} \label{x1bound}
		\Prob{\forall i \in \Istable : \infnorm{X_1} \le x} \ge 1 - 2ps\ex{-x^2/(2K^2\sigma^2_{\max})}
	\end{equation}
	
	Therefore, $\forall \ione, \itwo, \ithree, \ifour \in \{1,...,n\}$
	
	\begin{equation}
	\Prob{\forall i \in \Istable: \abs{X_{i,\ione} X_{i,\itwo} X_{i,\ithree} X_{i,\ifour} - \omega_{\ione, \itwo, \ithree, \ifour}}  \le x^4 + \abs{\omega_{\ione, \itwo, \ithree, \ifour}}} \ge 1 - 2ps\ex{-x^2/(2K^2\sigma^2_{\max})}
	\end{equation}
	
	By Bernstein inequality
	
	\begin{equation} \label{4mombern}
\begin{split}
	\Prob{\abs{\empE{X_{i,\ione} X_{i,\itwo} X_{i,\ithree} X_{i,\ifour}} - \omega_{\ione, \itwo, \ithree, \ifour}} \ge  \Bernstain{x^4+\abs{\omega_{\ione, \itwo, \ithree, \ifour}}}{t}{s}{\sigma^2_{4\max}}  } \\ 
	\le e^{-t}	
\end{split}
	\end{equation}
	
	And the combination of \eqref{4mombern} and \eqref{x1bound} establishes the claim.
	
\end{proof}

==> highProbabilitySetConditioning.tex <==
\begin{lemma}
	\label{pdfLemma}
	Let $x$ be a random variable and let $A$ be some set of probability $p_A>0$. Then
	
	\begin{equation}
	|\Prob{x < c} - \Prob{x < c | A} | \le 2(1-p_A)
	\end{equation}
	
\end{lemma}


\begin{proof}
	
	\begin{equation}
	\begin{split}
	|\Prob{x < c} - \Prob{x < c \given A} | &= |\Prob{x < c\ \given A} \Prob{A} + \Prob{x < c\ \given \overline A} \Prob{\overline A} - \Prob{x < c \given A} | \\
	& \le (1-p_A) \Prob{ x < c \given A } + \Prob{x < c\ \given \overline A} (1-p_A) \\
	& \le (1-p_A) + (1-p_A) \\
	& = 2(1-p_A)
	\end{split}
	\end{equation}
	
\end{proof}


==> pattern.tex <==
\subsection{Convolution with pattern}

Consider for a positive $n$ a sequence $\{P_n(i)\}_{i=1}^{2n}$ such that 

\begin{equation} \label{constitution}
\sum_{i=1}^{2n}\abs{P_n(i)} = 1 \text{ and } \sum_{i=1}^{2n}P_n(i) = 0
\end{equation}

and refer $P_n(\cdot)$ as pattern.

Also for a sequence of arbitrary length $\{a(k)\}_{k=1}^l \subset \R$ define convolution with pattern as an operation producing a vector with $l-2n+1$ components which are defined as

\begin{equation}
(a \star P)_j = \sum_{i=j}^{i=j+2n-1} a(i) P_n(i)
\end{equation}

Now we can define a pattern-convolved statistic as 

\begin{equation}
\patternA_n = A_n \star P
\end{equation}

\begin{equation}
\patternA = \max_{n \in \n} \infnorm{\patternA_n}
\end{equation}

The bootstrap procedure has to be augmented in a similar manner:


\begin{equation}
\patternAb_n = \Ab_n \star P
\end{equation}

\begin{equation}
\patternAb = \max_{n \in \n} \infnorm{\patternA_n}
\end{equation}

Finally, the critical level $\xalpha$ is suggested to be chosen as 

\begin{equation}
\Prob{\patternAb \le \xalpha} = 1-\alpha
\end{equation}

==> spokoinyLemma.tex <==
\begin{lemma}\label{mysplemma}
	Consider $\xi \sim \N{0}{\Sigma_\xi}$ and $\eta \sim \N{0}{\Sigma_\eta}$. Assume, in the sense of Loewner matrix ordering, $\Sigma_\eta \ge \Sigma_\xi$. Then for any $0$-centered $\ell_\infty$-ball $A$
	
	\begin{equation}
		\Prob{\xi \in A} \ge \Prob{\eta \in A}
	\end{equation}
\end{lemma}

\begin{proof}
	This result is trivial in a one-dimensional case. Higher-dimensional results are established by integration in polar coordinates.
\end{proof}
